Regret Balancing for Bandit and RL Model Selection

We consider model selection in stochastic bandit and reinforcement learning problems. Given a set of base learning algorithms, an effective model selection strategy adapts to the best learning algorithm in an online fashion. We show that by estimating the regret of each algorithm and playing the algorithms such that all empirical regrets are ensured to be of the same order, the overall regret balancing strategy achieves a regret that is close to the regret of the optimal base algorithm. Our strategy requires an upper bound on the optimal base regret as input, and the performance of the strategy depends on the tightness of the upper bound. We show that having this prior knowledge is necessary in order to achieve a near-optimal regret. Further, we show that any near-optimal model selection strategy implicitly performs a form of regret balancing.

==> experiments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bandit experiments}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bandit model selection experiments}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Reinforcement learning model selection experiments}


% Experiment 1 - Choosing the optimal discount factor: finite MDP, $M$ RL algorithms, the $i$th RL algorithm is a Q-learning method with discount factor $\gamma_i$. We set $\gamma_1=0$, $\gamma_M=0.99$, and some values in between. For $\gamma_1=0$, we are using a bandit algorithm. 

% Experiment 2 - Choosing between contextual bandits and RL: Given the state $x_t$ and action $a_t$, the next state is sampled according to an unknown transition dynamics $x_{t+1}\sim P(.|x_{t},a_{t})$. If $P(x'|x,a)=Q(x')$ for a distribution $Q$ independently of $(x,a)$, then a bandit algorithm might be appropriate. Otherwise, actions influence the distribution of the next states and an RL algorithm might be appropriate. 

% Experiment 3 - Choosing between different feature vectors. 


==> old.tex <==
\textbf{Algorithm - } Let $V_t = \sum_{k=1}^{t-1} x_k x_k^\top$ be the empirical covariance matrix. In round $t$, let $y_t = \arg\max_{x\in D} x^\top \widehat \theta_t$. This is an estimate of the value of the best action. For a constant $C$, let $b_t$ such that 
\begin{align}
\label{eq:emp_regret}
\frac{1}{y_t^\top V_t^{-1} y_t} (b_t - y_t^\top \widehat \theta_t) = \frac{C}{\sqrt{y_t^\top V_t^{-1} y_t}} \;.
\end{align}
Throughout the game, we play actions to ensure that the empirical regret of all actions are roughly the same. This means that for all actions $x\in D$,
\begin{align}
\label{eq:regret_matching}
\frac{1}{x^\top V_t^{-1} x} (b_t - x^\top \widehat \theta_t) = \frac{C}{\sqrt{y_t^\top V_t^{-1} y_t}} \;.
\end{align}

\textbf{Analysis - } First, we state a standard result from least-squares analysis: For an appropriate constant $\beta < C$, with high probability, for any $x\in D$,
\begin{align}
\label{eq:least-squares}
| x^\top (\widehat \theta_t - \theta_*) | \le \beta \sqrt{x^\top V_t^{-1} x} \;.
\end{align}
By \eqref{eq:emp_regret}, \eqref{eq:least-squares}, and definition of $y_t$, 
\begin{align}
\notag
b_t &= y_t^\top \widehat\theta_t + C \sqrt{y_t^\top V_t^{-1} y_t} \\
\notag
&\ge x_*^\top \widehat\theta_t + C \sqrt{y_t^\top V_t^{-1} y_t} \\
\label{eq:bt}
&\ge x_*^\top \theta_* + C \sqrt{y_t^\top V_t^{-1} y_t} - \beta \sqrt{x_*^\top V_t^{-1} x_*} \;.
\end{align}
Next, we show that $b_t \ge x_*^\top \theta_*$. Proof by contradiction. If $b_t < x_*^\top \theta_*$, then by \eqref{eq:regret_matching}, 
\begin{align*}
\frac{C}{\sqrt{y_t^\top V_t^{-1} y_t}} &= \frac{1}{x_*^\top V_t^{-1} x_*} (b_t - x_*^\top \widehat \theta_t)  \\ 
&< \frac{1}{x_*^\top V_t^{-1} x_*} (x_*^\top \theta_* - x_*^\top \widehat \theta_t) \\
&\le \frac{\beta}{\sqrt{x_*^\top V_t^{-1} x_*}} \;.
\end{align*}
Given $C > \beta$, we conclude that $C \sqrt{y_t^\top V_t^{-1} y_t} \ge \beta \sqrt{x_*^\top V_t^{-1} x_*}$, which by \eqref{eq:bt}, implies that $b_t \ge x_*^\top \theta_*$. 

By \eqref{eq:regret_matching} and \eqref{eq:least-squares},
\begin{align}
\label{eq:eqq1}
\frac{1}{x^\top V_t^{-1} x} (b_t - x^\top \theta_*) = \frac{C}{\sqrt{y_t^\top V_t^{-1} y_t}} + \frac{\beta}{\sqrt{x^\top V_t^{-1} x}} \;.    
\end{align}
Given $b_t \ge x_*^\top \theta_*$, \eqref{eq:least-squares} and \eqref{eq:eqq1},
\[
\frac{1}{x^\top V_t^{-1} x} (x_*^\top \theta_*  - x^\top \theta_* ) \le \frac{C}{\sqrt{y_t^\top V_t^{-1} y_t}} + \frac{\beta}{\sqrt{x^\top V_t^{-1} x}} \;.  
\]
Thus,
\begin{align*}
R(T) &= \sum_{t=1}^T (x_*^\top \theta_* - x_t^\top \theta_*) \\
&\le \sum_{t=1}^T \left( \beta \sqrt{x_t^\top V_t^{-1} x_t} +  \frac{C x_t^\top V_t^{-1} x_t}{\sqrt{y_t^\top V_t^{-1} y_t}} \right) \\
&\le \beta \sqrt{T \log T} + C \sqrt{T} \log T \;.
\end{align*}
In the last step, we used the fact that 
\[
\lambda_{\text{max}}(V_t) \le \text{trace}(V_t) \le T\,,
\]
and hence 
\[
\lambda_{\text{min}}(V_t^{-1}) = \frac{1}{\lambda_{\text{max}}(V_t)} \ge \frac{1}{T} \;.
\]
Thus, $y^\top V_t^{-1} y \ge 1/T$ for any $y\in D$. 

problem dependant bounds



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Multi-Armed Bandits}

Consider a multi-armed bandit problem. In round $t$, the learner choose action $i_t$ from a set of $K$ actions and observes a Bernoulli reward $r_t$ with mean value $\mu_{i_t}$. Let $i_*$ be the optimal action defined as $i_* = \arg\max_{i\in [K]} \mu_i$. 
\\
\\
\noindent\textbf{Algorithm - } Let $N_{i,t}$ be the number of times that action $i$ is played up to time $t$, and let $R_{i,t}$ be the total reward of this arm during these $N_{i,t}$ rounds. Let $\beta$ be an appropriate constant. In round $t$, let 
\[
j_t = \arg\max_{i\in [K]}\, \frac{R_{i,t}}{N_{i,t}} + \frac{\beta}{\sqrt{N_{i,t}}} \;.
\]
be the optimistic action. This is an estimate of the value of the best action. Let $b_t$ such that 
\begin{align}
\label{eq:emp_regret_k}
N_{j_t,t} b_t - R_{j_t,t} = \beta\sqrt{N_{j_t,t}} \;.
\end{align}
Define the empirical regret of action $i$ by
\[
\widehat G_{i,t} = N_{i,t} b_t - R_{i,t} \;.
\]
The true regret is denoted by $G_{i,t} = N_{i,t} \mu_* - R_{i,t}$. Throughout the game, we play actions to ensure that the empirical regret of all actions are roughly the same. To be more precise, in time $t$, we choose the action with the smallest empirical regret:
\[
i_t = \arg\min_i\, \widehat G_{i,t} \;.
\]
We update the statistics and repeat this step. The goal is to ensure that for these actions,
\begin{align}
\label{eq:regret_matching_k}
N_{i,t} b_t - R_{i,t} \approx \beta\sqrt{N_{j_t,t}} \;.
\end{align}
\\
\\
\noindent\textbf{Analysis - } First, notice that $b_t$ is an optimistic estimate of $\mu_*$: By \eqref{eq:emp_regret_k} and definition of $j_t$, 
\begin{align}
\notag
b_t &= \frac{R_{j_t,t}}{N_{j_t,t}} + \frac{\beta}{\sqrt{N_{j_t,t}}} \\
\notag
&\ge \frac{R_{*,t}}{N_{*,t}} + \frac{\beta}{\sqrt{N_{*,t}}} \\
\label{eq:bt_k}
&\ge \mu_*  \;.
\end{align}
Let $j_t=i$ be the action with the largest UCB index. Thus, for any other action $k$,
\[
b_t = \frac{R_{i,t}}{N_{i,t}} + \frac{\beta}{\sqrt{N_{i,t}}} > \frac{R_{k,t}}{N_{k,t}} + \frac{\beta}{\sqrt{N_{k,t}}} \;.
\]
It also holds that $\widehat G_{i,t} = \beta \sqrt{N_{i,t}}$. We consider different cases. By induction, we will show that the state of the system always satisfies the following conditions. 
\begin{itemize}
\item Condition (A): if the UCB index is $i$ and the empirical regret of action $k\neq i$ is no less than that of action $i$, then regret of $k$ is less than $\beta\max\{\sqrt{N_{k,t}}, \sqrt{N_{i,t}}\}+1$. The base of induction holds at time $t=1$.
\item Condition (B): for any arm $k$, the regret satisfies $G_{k,t} \le \beta \sqrt{t} + 1$. 
\end{itemize}
\noindent\textbf{Case 1: } \underline{$\widehat G_{k,t} < \widehat G_{i,t}$}. So we play action $k$ at time $t+1$. In this case, 
\[
G_{k,t} \le N_{k,t} b_t - R_{k,t}< N_{i,t} b_t - R_{i,t} = \beta\sqrt{N_{i,t}} \;.
\]

\noindent\textbf{Case 1.1: } \underline{$j_{t+1}=i$ and $\widehat G_{k,t+1} > \widehat G_{i,t+1}$}. We have that $\widehat G_{i,t+1} = \widehat G_{i,t} = \beta \sqrt{N_{i,t}}$. Also,
\[
G_{k,t+1} = N_{k,t+1} \mu_* - R_{k,t+1} = (N_{k,t}+1) \mu_* - (R_{k,t} + r_t) = G_{k,t} + \mu_* - r_t \le \beta\sqrt{N_{i,t}} + 1 \;.
\]
Thus, Condition (A) is still satisfied. 

\noindent\textbf{Case 1.2: } \underline{$j_{t+1}=k$ and $\widehat G_{k,t+1} > \widehat G_{i,t+1}$}. Trivially, $\widehat G_{i,t+1} < \widehat G_{k,t+1} = \beta\sqrt{N_{k,t+1}} = \beta\sqrt{N_{k,t}+1}$.

\noindent\textbf{Case 1.3: } \underline{$j_{t+1}=i$ and $\widehat G_{k,t+1} < \widehat G_{i,t+1}$}. Trivially, $\widehat G_{k,t+1} < \widehat G_{i,t+1} = \beta\sqrt{N_{i,t+1}} = \beta\sqrt{N_{i,t}}$.

\noindent\textbf{Case 1.4: } \underline{$j_{t+1}=k$ and $\widehat G_{k,t+1} < \widehat G_{i,t+1}$}. We have that $\widehat G_{k,t+1} = \beta \sqrt{N_{k,t+1}}$. Also,
\[
G_{i,t+1} = N_{i,t+1} \mu_* - R_{i,t+1} = N_{i,t} \mu_* - R_{i,t} = G_{i,t} < \widehat G_{i,t} = \beta \sqrt{N_{i,t}} \;.
\]
Notice that Condition (A) is still satisfied.

\noindent\textbf{Case 2: } \underline{$\widehat G_{i,t} < \widehat G_{k,t}$ and Condition (A) holds}. So we play action $i$ at time $t+1$. In this case, $G_{k,t} \le \beta\max\{\sqrt{N_{k,t}}, \sqrt{N_{i,t}}\}+1$.

\noindent\textbf{Case 2.1: } \underline{$j_{t+1}=i$ and $\widehat G_{k,t+1} > \widehat G_{i,t+1}$}. Because $i$ is the UCB index and is also played, $\widehat G_{i,t+1} = \beta \sqrt{N_{i,t+1}}=\beta \sqrt{N_{i,t}+1}$. We also have
\[
G_{k,t+1} = N_{k,t+1} \mu_* - R_{k,t+1} = N_{k,t} \mu_* - R_{k,t} = G_{k,t} < \beta\max\{\sqrt{N_{k,t}}, \sqrt{N_{i,t}}\}+1 \,,
\]
where the last step holds by Condition (A) applied at time $t$. Notice that Condition (A) still holds at time $t+1$.

\noindent\textbf{Case 2.2: } \underline{$j_{t+1}=i$ and $\widehat G_{k,t+1} < \widehat G_{i,t+1}$}. Trivially, $\widehat G_{k,t+1} < \widehat G_{i,t+1} = \beta\sqrt{N_{i,t+1}} = \beta\sqrt{N_{i,t}+1}$. 

\noindent\textbf{Case 2.3: } \underline{$j_{t+1}=k$ and $\widehat G_{k,t+1} > \widehat G_{i,t+1}$}. Trivially, $\widehat G_{i,t+1} < \widehat G_{k,t+1} = \beta\sqrt{N_{k,t+1}} = \beta\sqrt{N_{k,t}}$. 

\noindent\textbf{Case 2.4: } \underline{$j_{t+1}=k$ and $\widehat G_{k,t+1} < \widehat G_{i,t+1}$}. We have $\widehat G_{k,t+1} = \beta \sqrt{N_{k,t+1}} = \sqrt{N_{k,t}}$. We also have
\begin{align*}
G_{i,t+1} &= N_{i,t+1}\mu_* - R_{i,t+1} \\ 
&= (N_{i,t}+1)\mu_* - (R_{i,t}+r_t) \\
&= G_{i,t} + \mu_* - r_t  \\
&\le \widehat G_{i,t} + \mu_* - r_t  \\
&\le \beta\sqrt{N_{i,t}}+1 \;.
\end{align*}
Thus, Condition (A) is still satisfied. 

Given that Condition (B) is always satisfied, we get that the total regret is bounded by $\beta K \sqrt{T} + 1$.


\if0
Let $V_{j,t}$ be the total reward of base $j$ up to time $t$ in the rounds that base $j$ is played. Let $N_{j,t}$ be the number of rounds that base $j$ is played up to time $t$. Let $i = \arg\max_j V_{j,t}/N_{j,t}$. Assume the regret of the optimal base is $U(t)$ up to time $t$. Define $b_t$ such that
\[
N_{i,t} b_{t} - V_{i,t} = U(N_{i,t}) \;.
\]
Intuitively, $b_{i,t}$ is an upper bound estimate of the reward of the optimal arm. Define empirical regret of base $k$ by $\widehat R_{k,t} = N_{k,t} b_{t} - V_{k,t}$. Let $b^*$ be the mean reward of the optimal arm. The true regret of the base $k$ is $R_{k,t} = N_{k,t} b^* - V_{k,t}$. 

Our model selection algorithm plays arms such that all $\widehat R_{k,t}$ become as close as possible to each other. Then we have that for any base $k$,
\begin{equation}
\label{eq:matching}
N_{k,t} b_{t} - V_{k,t} = N_{i,t} b_{t} - V_{i,t} = U(N_{i,t}) \;.
\end{equation}

Next, we analyze the regret of the model selection algorithm. If $b_{t} \geq b^*$, then by \eqref{eq:matching}, for any base $k$,
\[
R_{k,t} = N_{k,t} b^* - V_{k,t} \le N_{k,t} b_{t} - V_{k,t} = U(N_{i,t}) \;.
\]
Next, we will show that $b_{t}$ doesn't get much smaller than the optimal arm value. Assume $b_{t} < b^*$. 
%let k be the optimal base index
Given that the optimal base satisfies the given regret bound, $N_{*,t} b^* - V_{*,t} \leq U(N_{*,t})$. Given that $b_{t} < b^*$, 
\begin{equation}
\label{eq:optbase}
N_{*,t} b_{t} - V_{*,t} < U(N_{*,t}) \;.
\end{equation}
By definition and regret matching, for any base $k$, $N_{k,t} b_{t} - V_{k,t} \approx N_{i,t} b_{t} - V_{i,t} = U(N_{i,t})$. Given that the algorithm matches all empirical regrets, we should have 
\begin{equation}
\label{eq:eq0}
N_{k,t} b_{t} - V_{k,t} \approx N_{*,t} b_{t} - V_{*,t}\qquad \rightarrow \qquad U(N_{*,t}) > U(N_{i,t}) \;.
\end{equation}

\textcolor{red}{This implies the best base has been "pulled" at least as many times as the best empirical base.}

On the other hand, by the regret guarantee for the optimal base,
\begin{equation}
\label{eq:eq1}
N_{*,t} (b^* - b_{t}) + N_{*,t} b_{t} - V_{*,t} \leq U(N_{*,t}) \;.
\end{equation}
By regret matching and definition of $b_t$, 
\[
N_{*,t} b_{t} - V_{*,t}  = N_{i,t} b_{t} - V_{i,t} = U(N_{i,t}) > 0 \;.
\]
Thus, by \eqref{eq:eq1},
\[
N_{*,t} (b^* - b_{t}) \leq U(N_{*,t}) \;.
\]
Thus, by \eqref{eq:eq0} and given that $U$ is concave,
\[
b^* - b_{t} \leq \frac{U(N_{*,t})}{N_{*,t}} < \frac{U(N_{i,t})}{N_{i,t}} \;.
\]
By definition of $b_t$ and regret matching (\textcolor{red}{For any k}), $b_{t} \approx (V_{k,t} + U(N_{i,t}))/N_{k,t}$, and so
\[
b^* - \frac{V_{k,t}}{N_{k,t}} < \frac{U(N_{i,t})}{N_{k,t}} + \frac{U(N_{i,t})}{N_{i,t}} \;.
\]
Thus, 
\begin{equation}
\label{eq:eq2}
N_{k,t} b^* - V_{k,t} < U(N_{i,t}) + \frac{N_{k,t} U(N_{i,t})}{N_{i,t}} \;.
\end{equation}
\textcolor{red}{For any $k$}
Because we want to match regrets, we play base $k$ as long as it holds that $N_{k,t} b_{t} - V_{k,t} < N_{i,t} b_{t} - V_{i,t} = U(N_{i,t})$ and stop playing $k$ (and increasing $N_{k,t}$) when 
\[
N_{k,t} b_{t} - V_{k,t} \leq N_{i,t} b_{t} - V_{i,t} = U(N_{i,t}) \;.
\]
At this point, 
\[
N_{k,t}( b_{t} - V_{k,t}/N_{k,t}) \leq N_{i,t} (b_{t} - V_{i,t}/N_{i,t}) \;.
\]
Given that $i$ is the empirically best base and $V_{i,t}/N_{i,t} \geq V_{k,t}/N_{k,t}$, we get that $N_{k,t} \leq N_{i,t}$. Thus, by \eqref{eq:eq2},
\[
N_{k,t} b^* - V_{k,t} < 2 U(N_{i,t}) \;.
\]
So any arbitrary base is always played so that its cumulative regret respects the regret rate of the optimal base. Overall, we get at most $2 M U(T)$ for the total regret.
\fi













Let $i=j_t$ be the optimistic base. Thus, for any other base $k$,
\[
b_t = \frac{R_{i,t}}{N_{i,t}} + \frac{ U(N_{i,t})}{N_{i,t}} > \frac{R_{k,t}}{N_{k,t}} + \frac{ U(N_{k,t})}{N_{k,t}} \;.
\]
It also holds that $\widehat G_{i,t} = U(N_{i,t})$. We will show that the state of the system always satisfies the following conditions. 
\begin{itemize}
\item Condition (A): if $i$ is the optimistic base and the empirical regret of base $k\neq i$ is no less than that of base $i$, then regret of $k$ is less than $\max\{U(N_{k,t}), U(N_{i,t})\}+1$. 
\item Condition (B): for any base $k$, the regret satisfies $G_{k,t} \le U(t) + 1$. 
\end{itemize}
We will prove by induction. The base of induction holds at time $t=1$. Assume the statement holds at time $t$, and let $i$ be the optimistic base at time $t$. We show that the statement also holds at time $t+1$. We consider two cases. In the first case, there exits a base with empirical regret less than that of the optimistic base. 

\noindent\textbf{Case 1: } \underline{$\widehat G_{k,t} < \widehat G_{i,t}$ for any base $k\neq i$}. If we play base $k$ at time $t+1$, then, 
\[
G_{k,t} = \sum_{\tau\in N_{k,t}} \mu_{*,\tau} - R_{k,t} \le N_{k,t} b_t - R_{k,t}< N_{i,t} b_t - R_{i,t} = U(N_{i,t}) \;.
\]

\noindent\textbf{Case 1.1: } \underline{$j_{t+1}=i$}. We have $b_{t+1}=b_t$ as base $i$ is not played at time $t+1$. The empirical regret of any base that is not played remains the same and we have $\widehat G_{i,t+1} = \widehat G_{i,t} = U(N_{i,t})$. Let $k$ be the base $k$ that is played at time $t+1$. If $\widehat G_{k,t+1} > \widehat G_{i,t+1}$, we have that
\[
G_{k,t+1} = \sum_{\tau\in N_{i,t+1}} \mu_{*,\tau} - R_{k,t+1} = \sum_{\tau\in N_{i,t+1}} \mu_{*,\tau} - (R_{k,t} + r_{t+1}) = G_{k,t} + \mu_{*,t+1} - r_{t+1} \le U(N_{i,t}) + 1 \;.
\]
Thus, Condition (A) is still satisfied.  

If $\widehat G_{k,t+1} < \widehat G_{i,t+1}$, then trivially $\widehat G_{k,t+1} < \widehat G_{i,t+1} = \widehat G_{i,t} =  U(N_{i,t})$.

\noindent\textbf{Case 1.2: } \underline{$j_{t+1}\neq i$}. Let $k$ be the base played at time $t+1$. Given that the data only for this base has changed, then we should have $j_{t+1}=k$ and $b_{t+1} > b_t$. If there is a base $k'$ such that $\widehat G_{k',t+1} > \widehat G_{i,t+1}$, then for any other base $j$, $\widehat G_{j,t+1} < \widehat G_{k',t+1} =  U(N_{k',t+1}) =  U(N_{k',t}+1)$.




\noindent\textbf{Case 1.2: } \underline{$j_{t+1}=k$ and $\widehat G_{k,t+1} > \widehat G_{i,t+1}$}. Trivially, $\widehat G_{i,t+1} < \widehat G_{k,t+1} = \beta U(N_{k,t+1}) = \beta U(N_{k,t}+1)$.

\noindent\textbf{Case 1.4: } \underline{$j_{t+1}=k$ and $\widehat G_{k,t+1} < \widehat G_{i,t+1}$}. We have that $\widehat G_{k,t+1} = \beta U(N_{k,t+1})$. Also,
\[
G_{i,t+1} = \sum_{\tau\in N_{i,t+1}} \mu_{*,\tau}- R_{i,t+1} = \sum_{\tau\in N_{i,t}} \mu_{*,\tau} - R_{i,t} = G_{i,t} < \widehat G_{i,t} = \beta U(N_{i,t}) \;.
\]
Notice that Condition (A) is still satisfied.
\\
\\
\noindent\textbf{Case 2: } \underline{$\widehat G_{i,t} < \widehat G_{k,t}$ and Condition (A) holds}. So we play action $i$ at time $t+1$. In this case, $G_{k,t} \le \beta\max\{ U(N_{k,t}), U(N_{i,t})\}+1$.

\noindent\textbf{Case 2.1: } \underline{$j_{t+1}=i$ and $\widehat G_{k,t+1} > \widehat G_{i,t+1}$}. Because $i$ is the UCB index and is also played, $\widehat G_{i,t+1} = \beta U(N_{i,t+1})=\beta U(N_{i,t}+1)$. We also have
\[
G_{k,t+1} = \sum_{\tau\in N_{k,t+1}} \mu_{*,\tau} - R_{k,t+1} = \sum_{\tau\in N_{k,t}} \mu_{*,\tau} - R_{k,t} = G_{k,t} < \beta\max\{U(N_{k,t}), U(N_{i,t})\}+1 \,,
\]
where the last step holds by Condition (A) applied at time $t$. Notice that Condition (A) still holds at time $t+1$.

\noindent\textbf{Case 2.2: } \underline{$j_{t+1}=i$ and $\widehat G_{k,t+1} < \widehat G_{i,t+1}$}. Trivially, $\widehat G_{k,t+1} < \widehat G_{i,t+1} = \beta U(N_{i,t+1}) = \beta U(N_{i,t}+1)$. 

\noindent\textbf{Case 2.3: } \underline{$j_{t+1}=k$ and $\widehat G_{k,t+1} > \widehat G_{i,t+1}$}. Trivially, $\widehat G_{i,t+1} < \widehat G_{k,t+1} = \beta U(N_{k,t+1}) = \beta U(N_{k,t})$. 

\noindent\textbf{Case 2.4: } \underline{$j_{t+1}=k$ and $\widehat G_{k,t+1} < \widehat G_{i,t+1}$}. We have $\widehat G_{k,t+1} = \beta U(N_{k,t+1}) = U(N_{k,t})$. We also have
\begin{align*}
G_{i,t+1} &= \sum_{\tau\in N_{i,t+1}} \mu_{*,\tau} - R_{i,t+1} \\ 
&= \sum_{\tau\in N_{i,t+1}} \mu_{*,\tau} - (R_{i,t}+r_t) \\
&= G_{i,t} + \mu_{*,t+1} - r_{t+1}  \\
&\le \widehat G_{i,t} + \mu_{*,t+1} - r_{t+1}  \\
&\le \beta U(N_{i,t})+1 \;.
\end{align*}
Thus, Condition (A) is still satisfied. 

Given that Condition (B) is always satisfied, we get that the total regret is bounded by $\beta M U(T) + 1$. 


==> unknown_regret.tex <==
\section{Regret matching without knowledge of the optimal regret}
\label{app:unknown_regret}

\begin{proof}[Proof of Lemma~\ref{lemma:unknown_regret}]
Let $i^*$ be the best arm. Let $k^*$ be the best base. Let $N_{i,T}$ denote the number of times arm $i$ is selected up to time $T$. Let $M_{k,T}$ denote the number of times base $k$ is selected up to time $T$. Let $\mu_i$ and $\widehat \mu_{i,t}$ denote the true mean and the empirical mean of arm $i$ at time $t$. Let $R_{k,t}$  and $G_{k,t}$ be the reward and regret of base $k$ up to time $t$. Let $\mathcal{M}$ be the number of bases and $K$ be the number of arms. 

The master algorithm is as follow: 
\begin{itemize}
    \item Pull each arm $\left(\frac{T\mathcal{M}}{K}\right)^{2/3}$ times
    \item For each time step $t = (TM)^{2/3}K^{1/3} +1, \dots, T$: 
    
    Let $j_t = \argmax_i \widehat \mu_{i,t} + \frac{1}{\sqrt{N_i,t}}$ and $b_t = \max_i \widehat \mu_{i,t} + \frac{1}{\sqrt{N_i,t}} = \widehat \mu_{j_t,t} + \frac{1}{\sqrt{N_{j_t},t}}$. Calculate the empirical regret of each base $k$ as follow:
    \begin{align}
        \widehat G_{k,t} = M_{k,t} \cdot b_t - R_{k,t}
    \end{align}
    Play base $k_t = \argmin_k \widehat G_{k,t}$
\end{itemize}
 The regret of from the first step is $(T\mathcal{M})^{2/3}K^{1/3}$. 
 
 Now we analyze the regret from the second step. The cumulative regret of base $k_t$ at time $t$ where it is selected is:
\begin{align}
&G_{k_t,t} \\
    &=M_{k_t,t} \cdot \mu_{i^*} - R_{k_t,t} \\
    &< M_{k_t,t} \cdot \left( \widehat \mu_{i^*,t} + \frac{1}{\sqrt{N_{{i^*},t}}}\right) - R_{k_t,t} \text{ because $\mu_{i^*} < \widehat \mu_{i^*,t} + \frac{1}{\sqrt{N_{{i^*},t}}}$ with prob $1-\epsilon$ by Hoeffding}  \\
     &\le M_{k_t,t} b_t - R_{k_t, t} \text{ by definition of $b_t$} \\
     &\le M_{k^*,t} b_t - R_{k^*, t} \text{ by definition of $k_t$} \\
     &= M_{k^*,t} \cdot \left( \widehat \mu_{j_t,t} + \frac{1}{\sqrt{N_{{j_t},t}}} \right) - R_{k^*,t} \text{ by definition of $b_t$} \\
     &< M_{k^*,t} \cdot \left( \mu_{j_t} + \frac{2}{\sqrt{N_{j_t,t}}} \right) - R_{k^*,t} \text{ because $\widehat \mu_{j_t,t} - \frac{1}{\sqrt{N_{j_t,t}}} < \mu_{j_t}$ with prob $1-\epsilon$ by Hoeffding} \\
     &< M_{k^*,t} \cdot \left( \mu_{i^*} + \frac{2}{\sqrt{N_{j_t,t}}} \right) - R_{k^*,t} \text{ because $\mu_{j_t} < \mu_{i^*}$} \\
     &< M_{k^*,t} \cdot \mu_{i^*} - R_{k^*,t} + \frac{M_{k^*,t}}{\sqrt{N_{j_t,t}}} \\
     & = G_{k^*,t}+ \frac{M_{k^*,t}}{\sqrt{N_{j_t,t}}} \\
     &< G_{k^*,t}+ T^{2/3}K^{1/3}\mathcal{M}^{-1/3} \text{ because $M_{k^*,t}\le t \le T$ and $N_{j_t,t} \ge \left(\frac{T\mathcal{M}}{K}\right)^{2/3}$ from the first step} \label{eq:one_base_reqret}
\end{align}
Let $T_k$ be the last time step where base $k$ is picked. Then the regret of the master at the second time step is:
\begin{align}
    &\sum_{k} G_{k,T} \\
    =&\sum_{k} G_{k,T_k} \text{ by definition of $T_k$}\\
    <&\sum_k (G_{k^*,T_k}+ T^{2/3}K^{1/3}\mathcal{M}^{-1/3})\text{ by Eq.~\ref{eq:one_base_reqret}}\\
   < &\sum_k (G_{k^*,T}+ T^{2/3}K^{1/3}\mathcal{M}^{-1/3} )\text{ because $T_k \le T$} \\
   = &\mathcal{M} (G_{k^*,T}+ T^{2/3}K^{1/3}\mathcal{M}^{-1/3})
\end{align}
Then the regret of the master for both time steps is at most
\begin{align}
   2T^{2/3}\mathcal{M}^{2/3}K^{1/3}  + \mathcal{M}\cdot G_{k^*,T}
\end{align}
If $G_{k^*, T}  = \Omega(T^{2/3}
K^{1/3}\mathcal{M}^{-1/3})$ then the regret of the master is the same as the best base. 
\end{proof}
